UP2You: Fast Reconstruction of Yourself from Unconstrained Photo Collections

We present UP2You, the first tuning-free solution for reconstructing high-fidelity 3D clothed portraits from extremely unconstrained in-the-wild 2D photos. Unlike previous approaches that require "clean" inputs (e.g., full-body images with minimal occlusions, or well-calibrated cross-view captures), UP2You directly processes raw, unstructured photographs, which may vary significantly in pose, viewpoint, cropping, and occlusion. Instead of compressing data into tokens for slow online text-to-3D optimization, we introduce a data rectifier paradigm that efficiently converts unconstrained inputs into clean, orthogonal multi-view images in a single forward pass within seconds, simplifying the 3D reconstruction. Central to UP2You is a pose-correlated feature aggregation module (PCFA), that selectively fuses information from multiple reference images w.r.t. target poses, enabling better identity preservation and nearly constant memory footprint, with more observations. We also introduce a perceiver-based multi-reference shape predictor, removing the need for pre-captured body templates. Extensive experiments on 4D-Dress, PuzzleIOI, and in-the-wild captures demonstrate that UP2You consistently surpasses previous methods in both geometric accuracy (Chamfer-15%, P2S-18% on PuzzleIOI) and texture fidelity (PSNR-21%, LPIPS-46% on 4D-Dress). UP2You is efficient (1.5 minutes per person), and versatile (supports arbitrary pose control, and training-free multi-garment 3D virtual try-on), making it practical for real-world scenarios where humans are casually captured. Both models and code will be released to facilitate future research on this underexplored task. Project Page: https://zcai0612.github.io/UP2You

==> combined_figs_tables/Tab_Shape_Pred_and_Tab_front_view.tex <==
\begin{minipage}{\textwidth}

\begin{minipage}[t]{0.48\textwidth}
    \makeatletter\def\@captype{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \resizebox{0.90\textwidth}{!}{
        \begin{tabular}{c|cc|cc|c|c}
        \bottomrule
             Num of   & \multicolumn{2}{c|}{\semantify} & \multicolumn{2}{c|}{\prompthmr} & \multirow{2}{*}{MLP} & \multirow{2}{*}{Ours}\\ \cline{2-5}
           References     &    \down{Mean$\downarrow$}   &   \down{Var$\downarrow$}    &    \down{Mean$\downarrow$}    &   \down{Var$\downarrow$}     &                                            \\ \cline{1-7}
        3  &   11.087  &   4.234  &   9.212    &   10.370  &   8.819   &   \textbf{7.967}                                    \\
        6  &   11.066  &   5.706  &   9.661    &   17.465  &   8.046   &   \textbf{7.427}                                    \\
        9  &   10.978  &   6.424  &   9.403    &   18.218  &   8.275   &   \textbf{7.403}                                    \\
        12 &   11.097  &   6.597  &   9.287    &   19.418  &   8.336   &   \textbf{7.399}                                    \\ \toprule
        
        \end{tabular}
    }
    \vspace{-1.0em}
    \caption{\scriptsize \textbf{V2V($\downarrow$) Comparions of Shape Prediction Reuslts.}}
    \label{tab:puzzle-to-shape}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
    \makeatletter\def\@captype{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \resizebox{0.98\linewidth}{!}{
        \begin{tabular}{c|ccc|ccc}
        \bottomrule
                  &   \up{PSNR$\uparrow$}  &   \up{SSIM$\uparrow$}   &   \down{LPIPS$\downarrow$}   &   \down{Chamfer$\downarrow$}  &   \down{P2S$\downarrow$}     &  \down{Normal$\downarrow$}  \\ \cline{1-7}
        PSHuman   &   24.134               &   0.905                 &   0.0895                     &   2.759                       &   2.926                      &  0.0189              \\
        Ours Mesh &   \textbf{26.651}               &   \textbf{0.935}                 &   \textbf{0.0527}                     &   \textbf{0.927}                       &   \textbf{0.949}                      &  \textbf{0.0096}              \\ \toprule
        
        
        \end{tabular}
    }
    \vspace{-1.0em}
    \caption{\scriptsize \textbf{Comparison of Single-Image based Reconstruction.}}
    \label{tab:compare_front_view}
\end{minipage}
\end{minipage}
\vspace{-0.5em}


==> tabs_rebuttal/pcfa_image_encoder_with_gama.tex <==
\begin{minipage}{\textwidth}
% \vspace{-0.5em}
\begin{minipage}[t]{0.48\textwidth}
    \makeatletter\def\@captype{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \resizebox{0.65\textwidth}{!}{
        \begin{tabular}{c|ccc}
        \bottomrule
                        &  \up{PSNR$\uparrow$}   &   \up{SSIM$\uparrow$}   &   \down{LPIPS$\downarrow$}  \\ \cline{1-4}
        \textbf{DINOv2} &   \textbf{25.848}      &   \textbf{0.920}        &   \textbf{0.0576}           \\
        CLIP            &   23.876               &   0.904                 &   0.0767                    \\
        DINOv1          &   24.170               &   0.907                 &   0.0745                    \\ \toprule
        \end{tabular}
    }
    \vspace{-0.5em}
    \caption{\scriptsize \textbf{Comparison of Different Image Encoders for PCFA.}}
    \label{tab:image_encoder_pcfa}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
    \makeatletter\def\@captype{table}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \resizebox{0.75\linewidth}{!}{
        \begin{tabular}{c|cccc}
        \bottomrule
                           &   \up{PSNR$\uparrow$}   &   \up{SSIM$\uparrow$}   &   \down{LPIPS$\downarrow$}  &  \down{GPU$\downarrow$}   \\ \cline{1-5}
        $\numfeat=1.0$     &   24.978                &   0.912                 &   0.0665                    &  \textbf{18.64}           \\ \rowcolor{gray!20}
        $\numfeat=2.0$     &   \textbf{25.848}       &   \textbf{0.920}        &   0.0576                    &  20.88                    \\  
        $\numfeat=3.0$     &   25.837                &   \textbf{0.920}        &   \textbf{0.0569}           &  23.12                    \\ \toprule
        \end{tabular}
    }
    \vspace{-0.5em}
    \caption{\scriptsize \textbf{Comparison of Different Number of Selected Features.}}
    \label{tab:num_feature_selected}
\end{minipage}
\end{minipage}


